MotionEditor: Editing Video Motion via Content-Aware Diffusion

Existing diffusion-based video editing models have made gorgeous advances for editing attributes of a source video over time but struggle to manipulate the motion information while preserving the original protagonist's appearance and background. To address this, we propose MotionEditor, a diffusion model for video motion editing. MotionEditor incorporates a novel content-aware motion adapter into ControlNet to capture temporal motion correspondence. While ControlNet enables direct generation based on skeleton poses, it encounters challenges when modifying the source motion in the inverted noise due to contradictory signals between the noise (source) and the condition (reference). Our adapter complements ControlNet by involving source content to transfer adapted control signals seamlessly. Further, we build up a two-branch architecture (a reconstruction branch and an editing branch) with a high-fidelity attention injection mechanism facilitating branch interaction. This mechanism enables the editing branch to query the key and value from the reconstruction branch in a decoupled manner, making the editing branch retain the original background and protagonist appearance. We also propose a skeleton alignment algorithm to address the discrepancies in pose size and position. Experiments demonstrate the promising motion editing ability of MotionEditor, both qualitatively and quantitatively.

==> sec/0_abstract.tex <==
\begin{abstract}
% Despite gorgeous advances in diffusion-based video editing, existing video editing models are only limited to editing attributes of source video over time. Most of the existing diffusion-based models struggle to edit the motion information of video while preserving the original protagonist's appearance and background information, while motion editing is rated as higher-level editing than attribute-based editing. In this paper, we propose MotionEditor to address this challenge. MotionEditor is based on Stable Diffusion and ControlNet. Concretely, we propose a novel temporal-latent aware adapter plugged into ControlNet for capturing temporal motion correspondences. We implement ControlNet to exploit the motion feature at the independent frame-wise level. However, ControlNet is derived from the image domain, resulting in temporal inconsistency. Our adapter complements the ControlNet by leveraging mutual layered frame-wise representations and layered motion representations to transfer disentangled motion information over each frame. Moreover, we built up a two-branch (reconstruction branch and editing branch) architecture. We then proposed an attention injection mechanism based on these two branches. It enables the editing branch to query the key and value from the reconstruction branch in a decoupled manner forcing the editing branch to retain the original background and protagonist appearance. Additionally, the poses between source and target always occur mismatching in terms of size and position.
% Consequently, we propose a skeleton alignment algorithm to tackle this problem. Extensive experiments demonstrate the promising motion editing ability of our MotionEditor in qualitative and quantitative views. To the best of our knowledge, MotionEditor is the first dedicated model to tackle video motion editing challenges.

Existing diffusion-based video editing models have made gorgeous advances for editing attributes of a source video over time but struggle to manipulate the motion information while preserving the original protagonist's appearance and background.
To address this, we propose MotionEditor, the first diffusion model for video motion editing.
MotionEditor incorporates a novel content-aware motion adapter into ControlNet to capture temporal motion correspondence.
While ControlNet enables direct generation based on skeleton poses, it encounters challenges when modifying the source motion in the inverted noise due to contradictory signals between the noise (source) and the condition (reference).
Our adapter complements ControlNet by involving source content to transfer adapted control signals seamlessly.
Further, we build up a two-branch architecture (a reconstruction branch and an editing branch) with a high-fidelity attention injection mechanism facilitating branch interaction. 
This mechanism enables the editing branch to query the key and value from the reconstruction branch in a decoupled manner, making the editing branch retain the original background and protagonist appearance.
We also propose a skeleton alignment algorithm to address the discrepancies in pose size and position.
Experiments demonstrate the promising motion editing ability of MotionEditor, both qualitatively and quantitatively.
To the best of our knowledge, MotionEditor is the first diffusion-based model capable of video motion editing.
More examples can be found at the anonymous website \url{https://motioneditor.github.io/}.

\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
% \xintong{Intro too long.}
Diffusion models~\cite{dhariwal2021diffusion,ho2020denoising,ho2022cascaded,nichol2021improved,song2020score,song2020denoising,rombach2022high,meng2021sdedit,hertz2022prompt,tumanyan2023plug} have achieved remarkable success in image generation, which inspired plenty studies in video editing~\cite{wu2023tune,liu2023video,qi2023fatezero,ceylan2023pix2video,khachatryan2023text2video}.
%in various generative tasks, including image editing~\cite{meng2021sdedit,hertz2022prompt,tumanyan2023plug} and video editing~\cite{liu2023video,qi2023fatezero,ceylan2023pix2video}.
%The impressive performance of image editing with diffusion models has inspired a plethora of work on video editing~\cite{liu2023video,qi2023fatezero,ceylan2023pix2video}. 
While significant progress has been made, existing diffusion models for video editing primarily focus on texture editing, such as attribute manipulation for protagonists, background editing, and style editing. 
The motion information, which stands out as the most unique and distinct feature when compared to images, is mostly ignored.
%However, the motion information in videos is considered the most unique and distinct feature compared to the image domain. 
This raises the question: Can we manipulate the motion of a video in alignment with a reference video?
%Could a text-to-image diffusion model edit the motion of the source video following the target video? 
In this paper, we attempt to explore a novel, higher-level, and more challenging video editing scenario---motion editing. 
Given a reference video and prompt, we aim to change the protagonist's motion in the source to match the reference video while preserving the original appearance.
%with the motion from the target video while preserving the appearance of the protagonist and background in the source video.

% Edited videos are expected to enjoy high-fidelity and temporal consistency while inheriting the original geometry structure. 

% Most of existing diffusion-based video editing models introduce additional temporal modeling ~\cite{wu2023tune} to the text-to-image diffusion~\cite{rombach2022high} and exploit various correlated contents (attention map~\cite{liu2023video, qi2023fatezero, ceylan2023pix2video, khachatryan2023text2video, wang2023zero}, optical flow~\cite{cong2023flatten}, condition representations~\cite{lee2023soundini, chen2023control, karim2023save, feng2023ccedit}) from original video. These video editing models have shown explicit enhancement of temporal-spatial consistency. Another video editing paradigm is to decompose the video semantics with the help of layered neural atlas~\cite{kasten2021layered, bar2022text2live, chai2023stablevideo}, and each atlas represents the target object waiting to be edited. 
% The positions of the spatial-temporal contents are mapped to corresponding 2D positions in each atlas layer forming 2D UV maps. 
% This decoupling paradigm can strictly preserve the geometry structure of the original objects in the source video.

% There are some existing text-to-image based diffusion models to handle image pose editing through prompt descriptions~\cite{cao2023masactrl}, user interactive points~\cite{shi2023dragdiffusion, mou2023dragondiffusion}, or implementing ControlNet~\cite{zhang2023adding} with additional skeleton conditions. However, they do not take temporal consistency into account, which presents temporal jittering when applied directly to the video domain. 
% Motion editing can be comprehended as a set of frame-wise pose editing with the consideration of temporal consistency. There are only a few motion-guided video generation models. 
% On the other hand, few motion-guided video generation models decompose video editing into a set of frame-wise pose editing with the consideration of temporal consistency.
% Follow Your Pose~\cite{ma2023follow} and ControlVideo~\cite{zhang2023controlvideo} both attempt to design a condition-based controllable adapter for motion-guided video generation, similar to the role of ControlNet~\cite{zhang2023adding} in the image domain. However, these methods only concentrate on generation instead of editing. They prioritize capturing motion signals while neglecting the preservation of the protagonist's appearance and the background in the original videos.

To date in literature, researchers have explored human motion transfer~\cite{liu2019liquid,siarohin2019first,siarohin2021motion} and pose-guided video generation~\cite{ma2023follow,zhang2023controlvideo}. The former focuses on animating still images based on reference skeletons, while the latter tries to generate pose-aligned videos without preserving a desired appearance.
Motion editing differs in that it directly modifies the motion in the video while preserving other video information, such as dynamic per-frame background and camera movements.
% Notably, motion editing differs from human motion transfer~\cite{liu2019liquid,siarohin2019first,siarohin2021motion}. 
% The former directly modifies the motion in the source video, leveraging reference video and prompt, while the latter animates the image based on reference skeletons.
% Motion editing requires preserving additional video information, such as dynamic background and camera movements. 
% Moreover, Pose-guided video generation only focuses on generation while ignoring the preservation of original video appearance information. 

%There are several existing diffusion models on image pose editing~\cite{cao2023masactrl, shi2023dragdiffusion, mou2023dragondiffusion, zhang2023adding} and pose-guided video generation~\cite{ma2023follow, zhang2023controlvideo}.
Recent advancements in visual editing have mainly emerged through the use of diffusion models~\cite{cao2023masactrl, shi2023dragdiffusion, mou2023dragondiffusion,zhang2023adding,ma2023follow,zhang2023controlvideo}.
For example, ControlNet~\cite{zhang2023adding} enables direct controllable generation conditioned on poses.
However, they suffer from severe artifacts when trying to edit the motion according to another pose.
We hypothesize the reason is that the control signals are only derived from the reference poses, which cannot properly accommodate the source content, thus resulting in a contradiction.
Some methods also lack the ability to preserve the appearance of the protagonist and background, as well as the temporal consistency. In this paper, we rethink the fundamental efficacy of ControlNet.
We argue that it is essential to involve the source latent when generating the controlling signal for the editing task. With the help of source contents, the condition guidance can precisely perceive the entire context and structures, and adjust its distribution to prevent undesired distortion.

To this end, we propose MotionEditor, depicted in Fig. \ref{fig:overview}, to take one step forward in exploring video motion editing with diffusion models. 
MotionEditor requires one-shot learning on a source video to preserve the original texture feature. 
%for tackling the misalignment problem between source skeleton and target skeleton.
We then introduce a content-aware motion adapter appended to ControlNet for enhancing control capability and temporal modeling.
%temporal modeling and motion modeling. 
% The adapter consists of temporal convolution, temporal self-attention, and skeleton-content cross-attention. Temporal convolution and temporal self-attention on skeletons tend to compensate for the lack of temporal modeling capability in ControlNet.
The adapter consists of content-aware blocks and temporal blocks.
In particular, content-aware blocks perform cross-attention to incorporate the source frame feature, which significantly boosts the quality of motion control.
%Content-aware blocks perform cross-attention between each skeleton representation and the corresponding frame-wise representation from the diffusion U-Net to enhance the motion constraint of the protagonist in each frame. 
%During one-shot training, source video and source skeletons are fed to MotionEditor. 
%The parameters of the adapter are trainable while the other parameters of diffusion are frozen.



At inference time, a skeleton alignment algorithm is devised to counter the size and position disparities between source skeletons and reference skeletons. We further propose an attention injection mechanism based on a two-branch architecture (reconstruction and editing branches) to preserve the source appearance of the protagonist and the background.
%we further propose an attention injection mechanism based on a two-branch architecture (a reconstruction branch and an editing branch) during inference. 
Previous attention fusion strategies directly inject the attention map or key into the editing branch. The direct injection may result in confusion between the edited foreground and background. 
In some cases, it would bring noise to the editing branch, thereby resulting in the phenomenon of overlapping and shadow flickering. 
To avoid this, we propose to decouple the keys/values in the foreground and background using a segmentation mask.
%propose a novel attention injection mechanism based on decoupling operations. Before attention injection, we implement an off-the-shelf person segmentation model to the source video to obtain the protagonist masks. 
% The masks can separate the foreground and background of the source video. 
The keys/values in the editing branch are thus supplemented by those from the foreground and background in the reconstruction branch.
%Concretely, we utilize source masks to decouple the keys and values into foreground and background in the reconstruction branch. 
%We then concatenate the foreground and background from the reconstruction branch with the keys and the values from the editing branch forming the new keys and values. 
%We replace the original keys and values with the above new keys and values in the editing branch. 
As such, the editing branch is able to capture the background details and the geometric structure of the protagonist from the source. 
% It is worth noting that corresponding keys and values both refer to the set of the current frame from the query, the frame before the current frame. It can implicitly inject smoother background information from the reconstruction branch to the editing branch and alleviate the motion overlapping shadow flickering problem.


% Our proposed MotionEdit requires two inputs referring to video latent and corresponding protagonist skeleton signals. Consequently, we implement OpenPose Detector~\cite{zhang2023adding} to the source video and target video for obtaining source skeleton signals and target skeleton signals. Due to the different sizes and coordinated positions of protagonists, these two signals always cause misalignment resulting in editing performance degradation. To tackle this problem, we propose a novel signals alignment algorithm. Each skeleton is aligned before being fed into the model. 

% Specifically, we leverage the masks of the corresponding protagonist from the source video and target video to calculate the average based on the coordinates with a value of 1 in the mask to obtain the center of each protagonist, which masks are obtained by implementing an off-the-shelf person segmentation model. We calculate the affine matrix based on the center offset vector between the source protagonist and target protagonist to achieve position alignment through translation. We then resize the target protagonist based on the rectangular area corresponding to the protagonist in the respective mask to align the size with the source protagonist.

% Specifically, we perform resize and translation operation on target skeletons with the guidance of masks which are obtained by implementing an off-the-shelf person segmentation model.

% We conduct the experiments on extensive motion-prompt pairs. The results show the qualitative and quantitative superiority of our proposed MotionEditor among alternative competitors. With the help of xFormers~\cite{xFormers2022} and Accelerator~\cite{accelerate}, MotionEditor can accomplish video motion editing within several minutes on an NVIDIA A100. 

In conclusion, our contributions are as follows:
(1)  We are the first to explore video diffusion models for motion editing, which is usually ignored by previous video editing works.
%video motion editing diffusion models by introducing temporal-aware and motion-aware modeling. %It provides a promising way for this higher-level video editing. We want to spark the community's considerable interest in video motion editing instead of current video attribute editing. 
(2) A novel content-aware motion adapter is proposed to enable the ControlNet to perform consistent and precise motion editing. % It grants ControlNet the privilege to capture temporal motion features and correlated video latent-motion features, which enhances its capability of video motion editing. 
% Moreover, we propose a novel skeleton alignment algorithm to normalize the source protagonist skeletons and target protagonist skeletons, which promotes the model to be more precise in motion editing. 
(3) We propose a high-fidelity attention injection mechanism that preserves the background information and the geometric structure of the protagonist from the source. The mechanism is only active during inference, making it training-free.
(4) We conduct experiments on in-the-wild videos, where the results show the superiority of our method compared with the state-of-the-art.



==> sec/4_method.tex <==
\section{Method}
\label{sec:method}



% In this section, we first give an overview in Sec.~\ref{sec: architecture_overview}. We then introduce two important components of MotionEditor in Sec.~\ref{sec: adapter} and Sec.~\ref{sec: attention_fusion}. Finally, we describe the skeleton signal alignment algorithm in Sec.~\ref{sec: skeleton_alignment}.

\subsection{Architecture Overview}
\label{sec: architecture_overview}

As illustrated in Fig. \ref{fig:overview}, MotionEditor is based on the commonly used T2I diffusion model (\emph{i.e.} LDM~\cite{rombach2022high}) and ControlNet~\cite{zhang2023adding}.
%Our proposed MotionEditor is based on Stable Diffusion~\cite{rombach2022high} and ControlNet~\cite{zhang2023adding}. 
We first inflate the spatial transformer in the U-Net of the LDM to a 3D transformer by appending a temporal self-attention layer.
We also propose Consistent-Sparse attention, described in Sec.~\ref{sec: attention_fusion}, to replace the spatial self-attention.
To achieve precise motion manipulation and temporal consistency, we design a content-aware motion adapter, operating on features from the U-Net and conditional pose information from the ControlNet. Following~\cite{wu2023tune}, we perform one-shot training to compute the weights for the temporal attention module and the motion adapter to reconstruct the input source video.

% % A content-aware motion adapter is devised and appended to the ControlNet to regulate the output for precise motion manipulation and temporal consistency.
% % The adapter also takes the latent feature from the U-Net as input.
% Following~\cite{wu2023tune}, the temporal attention and motion adapter require additional one-shot training to learn the knowledge for editing.
% During training, only the motion adapter and temporal attention in U-Net are trainable.


%4.1所有公式都不必要，vae部分应该放到sec.3
%Stable Diffusion and ControlNet are both derived from image domains lacking the capacity to perceive temporal motion. Consequently, we implement C-Sparse Attention and Temporal Attention to U-Net in the Stable diffusion for adaption of the video domain. 
%The keys and values of the $i$-th frame contain the previous frame $\mathbf{f}_{i-1}$ and current frame $\mathbf{f}_{i}$ enabling the model to synthesize temporal consistency contents. 
%We then propose a Temporal-Latent-aware motion adapter to grant ControlNet the privilege to capture temporal motion representations, which the adapter is inserted into the bottom of ControlNet. 
% To preserve the original appearances during motion editing, we propose two stream attention injection mechanisms executed in the decoder parts. 
% There always exists a discrepancy in coordinate position and size between the source video protagonist and the target video protagonist. Therefore, we further propose a skeleton alignment algorithm for normalizing skeleton signals. 
%The architecture overview is illustrated in Figure \ref{fig:overview}. Our proposed motion adapter requires additional one-shot learning for learning the knowledge to fit the distribution of corresponding motion and background information. During the training process, the parameters of the motion adapter are trainable while the rest of the parameters are frozen. 

During inference, given a reference target video $\bm{X}_{rf}$, MotionEditor aims to transfer the motion of $\bm{X}_{rf}$ to the source while preserving the appearance information of the source.
To this end, we first develop a skeleton alignment algorithm to narrow the gap between source skeleton $\bm{S}_{sr}$ and reference skeleton $\bm{S}_{rf}$ by considering the position and size, and 
produce a refined target skeleton $\bar{\bm{S}}_{tg}$.
We then employ the DDIM inversion~\cite{song2020denoising} on pixel values of the video to produce a latent noise that serves as the starting point for sampling.
%Given source video $\mathbf{V}_{s}$ and target video $\mathbf{V}_{t}$, MotionEditor can transfer the motion of the target video to the source video while preserving the protagonist appearance and background of source video during the inference process. 
% The concrete motion editing process is depicted as follows: First, we implement OpenPose Detector~\cite{cao2017realtime} on the source video and target video to obtain corresponding skeletons. To narrow the gap between the source protagonist and the target protagonist, we utilize our proposed algorithm to align target skeletons to source skeletons:
% \begin{equation}\small
% \label{eq:overview_alignment}
% \begin{aligned}
%      \bar{\mathbf{S}}_{t} = \mathtt{Align}(\mathtt{OpenPose}(\mathbf{V}_{s}), \mathtt{OpenPose}(\mathbf{V}_{t})),
% \end{aligned}
% \end{equation}
% where $\bar{\mathbf{S}}_{t}$ refers to aligned target skeletons and $\mathtt{Align}(\cdot)$ refers to our proposed alignment algorithm. 
% Second, we implement VAE Encoder to the source video to transfer pixel values to latent space. To incorporate structure guidance from the source video, we utilize an inversion operation on latent space obtaining $\mathbf{X}_{T}$:
% \begin{equation}\small
% \label{eq:overview_inversion}
% \begin{aligned}
%      \mathbf{X}_{T} = \mathtt{Inversion}(\mathtt{Encoder_{vae}}(\mathbf{V}_{s})),
% \end{aligned}
% \end{equation}
% where $\mathtt{Encoder_{vae}}(\cdot)$ refers to Vae Encoder. 
More importantly, we introduce a high-fidelity attention injection module exploring a carefully designed two-branch network. One is dedicated to reconstruction, while the other one focuses on editing. More specifically, the editing branch takes features from the refined target skeleton as inputs, transferring the motion information from the reference to the source. Meanwhile, critical appearance information encoded in the reconstruction branch is further injected into the editing branch so that the appearance and the background are preserved. Below, we introduce the proposed components in detail.


% The motion feature from the adapter is injected into the editing branch. Moreover, a high-fidelity attention injection mechanism is designed to preserve the source appearance.
% This mechanism involves injecting the key and value from the reconstruction branch into the editing branch.
% Finally, we obtain the synthesized video from the editing branch.



%Third, we build two-stream architecture on $\mathbf{X}_{T}$ for reconstruction and motion editing. 
% We store the feature list $\mathbf{f}_{list}$ of the U-Net encoder in the editing branch for subsequent calculation of the motion adapter. 
% Meanwhile, we feed the aligned target skeletons to ControlNet $\mathtt{Control}$ for extracting condition features in the spatial view. 
% The stored feature list and the output of ControlNet are both sent to motion adapter $\mathtt{{A}_{m}}$ for further temporal-latent aware motion modeling: 
% \begin{equation}\small
% \label{eq:overview_adapter}
% \begin{aligned}
%      \mathbf{m}_{t} = \mathtt{A_{m}}(\mathtt{Control}(\mathbf{S}_{t}, \mathbf{P}_{t}), \mathtt{Enc_{edit}}(\mathbf{X}_{T}, \mathbf{P}_{t})),
% \end{aligned}
% \end{equation}
% where $\mathtt{Enc_{edit}}$ refers to U-Net encoder in the editing branch and $\mathbf{P}_{t}$ refers to target text prompts. $\mathbf{m}_{t}$ indicates the target motion representations derived from motion adapter. 
% In the end, we perform our proposed mutual attention injection mechanism to preserve the original protagonist appearance and background information. Concretely, we replace the keys and values of the editing branch with the corresponding keys and values of the reconstruction branch. 
% It is worth noting that each key and value corresponds to the previous frame $\mathbf{f}_{i-1}$ and the current frame $\mathbf{f}_{i}$ as the current frame index is $i$. 
% $\mathbf{m}_{t}$ is added to the inputs of the U-Net decoder in the editing branch for motion guidance:
% \begin{equation}\small
% \label{eq:overview_reconstruction}
% \begin{aligned}
%      \mathbf{V}_{r} = \mathtt{Dec_{rec}}(\mathtt{Enc_{edit}}(\mathbf{X}_{T}, \mathbf{P}_{s})),
% \end{aligned}
% \end{equation}

% \begin{equation}\small
% \label{eq:overview_reconstruction}
% \begin{aligned}
%      \mathbf{V}_{e} = \mathtt{Dec_{edit}}(\mathtt{Enc_{edit}}(\mathbf{X}_{T}, \mathbf{P}_{t})+\mathbf{m}_{t}, \mathbf{P}_{t}),
% \end{aligned}
% \end{equation}
% where $\mathbf{V}_{r}$ and $\mathbf{V}_{e}$ refer to reconstructed video and motion edited video respectively. We denote $\mathbf{P}_{s}$, $\mathtt{Dec_{rec}}$, $\mathtt{Dec_{edit}}$ as source text prompts, reconstruction branch U-Net decoder and editing branch U-Net decoder respectively. 

\subsection{Content-Aware Motion Adapter}
%Temporal-Latent-Aware Motion Adapter
\label{sec: adapter}
Our goal is to manipulate the body motion in videos under the guidance of pose signals.
While ControlNet~\cite{zhang2023adding} enables direct controllable generation based on conditions, it has difficulties modifying the source motion from the inverted noise.
The motion signals injected by the ControlNet could conflict with the source motion, thereby resulting in pronounced ghosting and blurring effects or even the loss of controlling ability.
Furthermore, the model is derived from an image, lacking the ability to generate temporal consistent contents.
%ControlNet~\cite{zhang2023adding} enables Stable Diffusion to learn additional given conditions resulting in synthesizing controllable diverse contents. However, ControlNet is derived from the image domain lacking the ability to generate temporal consistency contents. 
Therefore, we propose a temporal content-aware motion adapter that enhances motion guidance as well as facilitates temporal consistency, as shown in Fig. \ref{fig:overview}.
%Therefore, we propose a temporal-latent-aware motion adapter to enable ControlNet to be sensitive to temporal motion and further enhance the strength of motion guidance. The structure of the motion adapter is depicted in the lower right corner of Figure \ref{fig:overview}. 

Our motion adapter takes as input the feature output by ControlNet, which has been observed to achieve promising spatial control.
Instead of inserting temporal layers into ControlNet, we leave it as is to prevent prejudicing its inherent modeling capability.
The adapter consists of two parallel paths corresponding to different perception granularity.
One is the global modeling path, including a content-aware cross-attention block and a temporal attention block. The other is the local modeling path, which uses two temporal convolution blocks to capture local motion features.
Specifically, our cross-attention involves the latent feature from the U-Net to model the pose feature, where the query comes from the pose feature $\bm{m}_{i}$, and the key/value is from the corresponding frame latent $\bm{z}_{i}$ produced by the U-Net:
%Motion adapter consists of temporal convolution, temporal self-attention, and cross attention between skeleton representations and video latent. 
%Extensive experiments have demonstrated that ControlNet has promising controllable pose modeling capacity in the spatial view. 
%Video motion can be comprehended as the collection of variable poses with temporal consistency. Therefore, we choose to directly leverage the output of the ControlNet as the input of our motion adapter instead of the original raw skeletons. 
%We divide the input data stream into two streams for modeling levels of different granularity. For the local modeling stream, we utilize temporal convolution with residual connection to capture local motion features. 
%For the global modeling stream, we first design a latent-aware cross-attention. Concretely, we derive a query from current $i$-th frame motion feature $\mathbf{motion}_{i}$, key and value from corresponding frame latent feature $\mathbf{l}_{i}$ in the editing branch. The $\mathtt{Cross-Attention}(\mathbf{Q},\mathbf{K},\mathbf{V})=\mathtt{Softmax}(\frac{\mathbf{Q}\mathbf{K}^{T}}{\sqrt{d}}\cdot \mathbf{V} )$ is calculated with:
\begin{equation}\small
\label{eq:overview_cross_attn}
\begin{aligned}
     \bm{Q}=\bm{W}_c^{Q}\bm{m}_{i},\bm{K}=\bm{W}_c^{K}\bm{z}_{i},\bm{V}=\bm{W}_c^{V}\bm{z}_{i},
\end{aligned}
\end{equation}
where {\small$\bm{W}_c^{Q}$, $\bm{W}_c^{K}$} and {\small$\bm{W}_c^{V}$} are projection matrices.
Our cross-attention enables the motion adapter to concentrate on correlated motion clues in the video latent space, which significantly enhances the control capability.
By building up a bridge between them, the model can thereby manipulate the source motion seamlessly, without contradiction.
%We then utilize temporal self-attention for global temporal modeling after building up latent-aware relationships. In the end, we fuse two streams by adding an operation.




\subsection{High-Fidelity Attention Injection}
%Content-Consistent Attention Injection}
%Two Stream Attention Injection Mechanism}
\label{sec: attention_fusion}

Although our motion adapter can accurately capture body poses, it may undesirably alter the appearance of the protagonist and the background.
%capture temporal-latent aware motion representations, it may change the original protagonist's appearance and background information inevitably during motion transferring. 
Consequently, we propose a high-fidelity attention injection from the reconstruction branch to the editing branch, which preserves the details of the subject and background in the synthesized video.
%based on two stream frameworks (reconstruction branch and editing branch). 
%Our proposed mechanism can inject global and local correlated representations from the reconstruction branch to the editing branch which enables the editing branch to preserve the original appearance and background information. 
While previous attention fusion paradigms~\cite{qi2023fatezero,wang2023zero,cao2023masactrl} have used attention maps or keys/values for editing, they suffer from severe quality degradation in ambiguous regions, \ie motion areas, due to context confusion.
%Unlike the previous attention fusion paradigm in video editing~\cite{qi2023fatezero, khachatryan2023text2video, wang2023zero}, we only take key and value from the reconstruction branch into consideration instead of the whole attention map. 
To solve the issue, we decouple the keys and values into foreground and background through semantic masks.
By injecting separated keys and values into the editing branch from the reconstruction branch, we can reduce the confusion hindering the editing.
%In order to prevent the foreground and background information from mixing with each other and interfering with the attention query operation, we semantically decouple key and value through masks, which we leverage masks to decouple and separate the background and foreground in key and value. 
%We will inject the decoupled keys and values into the editing branch as a new key and value. 
The pipeline is shown in Fig. \ref{fig:attention}.


\begin{figure}[t!]
\begin{center}
\includegraphics[width=1\linewidth]{attention.pdf}
\end{center}
\vspace{-0.6cm}
   \caption{Illustration of high-fidelity attention injection during inference. We leverage the source foreground masks to guide the decoupling of key/value in the Consistent-Sparse Attention.}
\label{fig:attention}
\vspace{-0.4cm}
\end{figure}


% Our injection mechanism leverages the keys and values in the reconstruction branch to complement those in the editing branch. The mechanism is active in the decoder.
%operates on the decoder of the U-Net.
Before introducing the injection, we first present the details of attention blocks in the model.
Each attention block in U-Net consists of our designed Consistent-Sparse Attention (CS Attention), Cross Attention, and Temporal Attention. 
%Our injection mechanism operates on the C-Sparse Attention Blocks and Temporal Attention Blocks of the U-Net decoder. U-Net decoder of MotionEditor is consisted with C-Sparse Attention, Cross Attention and Temporal Attention. 
The Consistent-Sparse Attention, as a sparse causal attention, replaces the spatial attention in the original U-Net.
It aims to perform spatiotemporal modeling with little additional computational overhead.
%performs slightly differently in the two branches. 
Specifically, taking the reconstruction branch as an example, the query in CS Attention is derived from the current frame $\bm{z}^r_{i}$, while the key/value is obtained from the preceding and current frames $\bm{z}^r_{i-1},\bm{z}^r_{i}$. 
This design can improve the frame consistency:
\begin{equation}\small
\label{eq:attention_sparse}
\begin{aligned}
     \bm{Q}^r=\bm{W}^{Q}\bm{z}^r_{i},\bm{K}^r=\bm{W}^{K}[\bm{z}^r_{i-1}, \bm{z}^r_{i}],\bm{V}^r=\bm{W}^{V}[\bm{z}^r_{i-1}, \bm{z}^r_{i}],
\end{aligned}
\end{equation}
where $[\cdot]$ refers to concatenation. {\small$\bm{W}^{Q}$, $\bm{W}^{K}$} and {\small$\bm{W}^{V}$} are projection matrices.
% this paragraph must be after the introduction of cs attn
It is worth noting that we do not employ the sparse attention in~\cite{wu2023tune}, in which the key/value is from the first and preceding frames $\bm{z}_{0},\bm{z}_{i-1}$.
We find that it may force the synthesized motion to favor the first frame excessively, resulting in flickering.

%It is worth noting that we do not utilize previous Sparse Attention~\cite{wu2023tune} which derives query features from current frame $\mathbf{f}_{i}$, key and value features from the first frame $\mathbf{f}_{0}$ and the former frame $\mathbf{f}_{i-1}$. We find that the previous Sparse Attention~\cite{wu2023tune} may force the synthesized motion to excessively favor the first frame resulting in flickering. 
%To address this problem, we propose Consistent-Sparse Attention (C-Sparse Attention) which derives query features from current frame $\mathbf{f}_{i}$, key and value features from the former frame $\mathbf{f}_{i-1}$ and the current frame $\mathbf{f}_{i}$. 
% We implement C-Sparse Attention $\mathtt{Attention}(\mathbf{Q},\mathbf{K},\mathbf{V})$ with
% \begin{equation}\small
% \label{eq:attention_sparse}
% \begin{aligned}
%      \mathbf{Q}={W}^{Q}\mathbf{f}_{i},\mathbf{K}={W}^{K}[\mathbf{f}_{i-1}, \mathbf{f}_{i}],\mathbf{V}={W}^{V}[\mathbf{f}_{i-1}, \mathbf{f}_{i}]
% \end{aligned}
% \end{equation}
% where $[\cdot]$ refers to concatenation operation. $W^{Q}$, $W^{K}$ and $W^{V}$ are projection matrices.


We now present the injection of keys and values from the reconstruction branch to those of the editing branch, operating on both Consistent-Sparse Attention (CS Attention) and Temporal Attention. The injection is only active in the decoder of U-Net. For CS Attention, we leverage a source foreground mask {\small$\bm{M}$}, obtained from an off-the-shelf segmentation model, to decouple the foreground and background information.
Given the key {\small$\bm{K}^r$} and value {\small$\bm{V}^r$} in the reconstruction branch, we separate them into the foreground ({\small$\bm{K}^{r}_{fg}$} and {\small$\bm{V}^{r}_{fg}$}) and background ({\small$\bm{K}^{r}_{bg}$} and {\small$\bm{V}^{r}_{bg}$}),
%In terms of the Attention Injection Mechanism in C-Sparse Attention, we first implement an off-the-shelf person segmentation model on the source video obtaining source mask $\mathbf{M}_{s}$. Given the reconstruction branch key $\mathbf{K}_{r}$ and value $\mathbf{V}_{r}$, we leverage $\mathbf{Mask}_{s}$ to decouple $\mathbf{K}_{r}$ and $\mathbf{V}_{r}$ into foreground ($\mathbf{K}_{s}^{fg}$ and $\mathbf{K}_{s}^{bg}$) and background ($\mathbf{V}_{s}^{fg}$ and $\mathbf{V}_{s}^{bg}$):
\begin{equation}\small
\label{eq:attention_decouple}
\begin{aligned}
     \bm{K}^r_{fg}&=\bm{K}^r\odot \bm{M}, ~~\bm{V}^r_{fg}=\bm{V}^{r}\odot \bm{M}, \\
     \bm{K}^{r}_{bg}&=\bm{K}^{r}\odot (\bm{1}-\bm{M}), ~~\bm{V}^{r}_{bg}=\bm{V}^{r}\odot (\bm{1}-\bm{M}).
\end{aligned}
\end{equation}
The decoupling operation introduces an explicit distinction between background and foreground. It encourages the model to focus more on the individual appearance instead of mixing both, ensuring the high fidelity of the subject and background.
%The decouple operation can alleviate interference from source video motion as the separated background features and foreground features encourage the model to pay more attention to the source background and protagonist appearance instead of the original motion itself. 
%This decoupling paradigm allows the model to focus only on modeling the background or protagonist of the source video at one time instead of mixing both simultaneously. 
Notably, simply replacing the key/value in the editing branch with the above ones would cause a large number of abrupt motion changes, as the model is significantly influenced by the source motion.
Instead, we combine them to maintain the target motion precisely.
%Second, we introduce editing branch key and value to the attention fusion process, which can preserve target motion information. Simply replacing the key and value will cause the model to be influenced by the original video motion resulting in a large number of abrupt motion changes in the edited results. 
Therefore, in the editing branch, the key and value of CS Attention are updated by the injected key {\small$\bm{K}_{inj}$} and value {\small$\bm{V}_{inj}$}:
%the injected key {\small$\bm{K}_{inj}$} and value {\small$\bm{V}_{inj}$} for CS attention layer can be described as:
%we concatenate editing branch key $\mathbf{K}_{e}$ with $\mathbf{K}_{s}^{fg}$ and $\mathbf{K}_{s}^{bg}$ to acquire the mutual key $\mathbf{K}_{fuse}$. The operation of Value is the same as above. The process is described as:
\begin{equation}\small
\label{eq:attention_decouple}
\begin{aligned}
     &\bm{K}^{e} = \bm{W}^{K}[\bm{z}^e_{i-1},\bm{z}^e_{i}] = [\bm{W}^{K}\bm{z}^e_{i-1},\bm{W}^{K}\bm{z}^e_{i}]\mathrel{\coloneqq} [\bm{K}^{e}_{pr},\bm{K}^{e}_{cu}], \\
     %&\bm{K}^{e}_{cu}\mathrel{\coloneqq} \bm{W}^{K}\bm{z}^e_{i},~\bm{K}^{e}_{pr}\mathrel{\coloneqq} \bm{W}^{K}\bm{z}^e_{i-1}, \\
     &\bm{V}^{e} = \bm{W}^{V}[\bm{z}^e_{i-1},\bm{z}^e_{i}] = [\bm{W}^{V}\bm{z}^e_{i-1},\bm{W}^{V}\bm{z}^e_{i}]\mathrel{\coloneqq} [\bm{V}^{e}_{pr},\bm{V}^{e}_{cu}], \\
     %&\bm{V}^{e}_{cu}\mathrel{\coloneqq} \bm{W}^{V}\bm{z}^e_{i},~\bm{V}^{e}_{pr}\mathrel{\coloneqq} \bm{W}^{V}\bm{z}^e_{i-1}, \\
     &\bm{K}_{inj}=[\bm{K}^{r}_{fg}, \bm{K}^{r}_{bg}, \bm{K}^{e}_{cu}], \\
     &\bm{V}_{inj}=[\bm{V}^{r}_{fg}, \bm{V}^{r}_{bg}, \bm{V}^{e}_{cu}],
\end{aligned}
\end{equation}
where $\bm{z}^e_{i},\bm{z}^e_{i-1}$ indicate the current and preceding frames in the editing branch. {\small$\bm{K}^{e},\bm{V}^{e}$} are the original key and value in CS attention of the editing branch. {\small$\bm{K}^{e}_{cu},\bm{V}^{e}_{cu}$} are the key and value from the current frame.
%where we denote $\mathbf{K}_{e}^{cur}$ as the specific key corresponding to the current frame. Third, we replace the original $\mathtt{Attention}(\mathbf{Q}_{e},\mathbf{K}_{e},\mathbf{V}_{e})$ with $\mathtt{Attention}(\mathbf{Q}_{e},\mathbf{K}_{fuse},\mathbf{V}_{fuse})$ for mutual attention injection in the C-Sparse Attention Blocks.

The injection in temporal attention is much simpler than in CS Attention since it already performs the local operation concerning the spatial region.
We directly inject the {\small$\bm{K}^{r},\bm{V}^{r}$} of reconstruction branch into the editing branch.

%In terms of the Attention Injection Mechanism in Temporal Attention, it is not necessary to perform a decoupling operation on key and value as Temporal Attention is fine-grained level modeling. We just directly replace the original $\mathtt{Attention}(\mathbf{Q}_{e},\mathbf{K}_{e},\mathbf{V}_{e})$ with $\mathtt{Attention}(\mathbf{Q}_{e},\mathbf{K}_{r},\mathbf{V}_{r})$ for attention injection in the Temporal Attention Blocks.



% \begin{algorithm}[t!]
% \caption{Skeleton Alignment}
% \label{alg:alignment}
% \begin{algorithmic}
% \small 
% \State \textbf{Input:} Source Skeleton $\bm{S}_{sr}$, Source Mask $\bm{M}_{sr}$; Reference Skeleton $\bm{S}_{rf}$, Reference Mask $\bm{M}_{rf}$ \\
% \\
%  % $\triangleright$ OpenPose Detection and Protagonist Segmentation \\
%  % $\mathbf{S}_{s}=\mathtt{OpenPose}(\mathbf{V}_{s}), \mathbf{S}_{t}=\mathtt{OpenPose}(\mathbf{V}_{t})$ \\
%  % $\mathbf{Mask}_{s}=\mathtt{Seg}(\mathbf{V}_{s}), \mathbf{Mask}_{t}=\mathtt{Seg}(\mathbf{V}_{t})$ \\
%  % \\
%  $\triangleright$ Resize Operation 
%  \State $({x}_{s}, {y}_{s}), {h}_{s}, {w}_{s}=\mathtt{Rectangle}\_\mathtt{Boundary}(\bm{M}_{sr})$ 
%  \State $({x}_{r}, {y}_{r}), {h}_{r}, {w}_{r}=\mathtt{Rectangle}\_\mathtt{Boundary}(\bm{M}_{rf})$ 
%  \State $\bm{P}_{S}=\mathtt{resize}(\bm{S}_{rf}[~{y}_{r}:{y}_{r}+{h}_{r},{x}_{r}:{x}_{r}+{w}_{r}~], ({h}_{s}, {w}_{s}))$
%  \State $\bm{P}_{M}=\mathtt{resize}(\bm{M}_{rf}[~{y}_{r}:{y}_{r}+{h}_{r},{x}_{r}:{x}_{r}+{w}_{r}~], ({h}_{s}, {w}_{s}))$
%  \State $\bm{S}_{rf}=\mathtt{zeros} \textunderscore \mathtt{like}(\bm{S}_{sr})$ 
%  \State $\bm{M}_{rf}=\mathtt{zeros} \textunderscore \mathtt{like}(\bm{M}_{sr})$ 
%  \State $\bm{S}_{rf}[~{y}_{s}:{y}_{s}+{h}_{s},{x}_{s}:{x}_{s}+{w}_{s}~]=\bm{P}_{S}$ 
%  \State $\bm{M}_{rf}[~{y}_{s}:{y}_{s}+{h}_{s},{x}_{s}:{x}_{s}+{w}_{s}~]=\bm{P}_{M}$ 
% \\
% \State $\triangleright$ Translation Operation
% % \State $\mathbf{Coordinates}_{s}=\mathtt{Argwhere}(\mathbf{M}_{s}==1)$
% % \State $\mathbf{Coordinates}_{t}=\mathtt{Argwhere}(\mathbf{M}_{t}==1)$
% \State $\mathbf{coordinates}_{s}=\mathtt{where}(\bm{M}_{sr}==1)$
% \State $\mathbf{coordinates}_{r}=\mathtt{where}(\bm{M}_{rf}==1)$
% \State $\mathbf{center}_{s}=\mathtt{Mean}(\mathbf{coordinates}_{s}, \mathtt{axis}=0)$
% \State $\mathbf{center}_{r}=\mathtt{Mean}(\mathbf{coordinates}_{r}, \mathtt{axis}=0)$
% \State $\bm{v}_{trans}=\mathbf{center}_{s}-\mathbf{center}_{r}$
% \State ${dx}=\bm{v}_{trans}~[~0~],~~{dy}=\bm{v}_{trans}~[~1~]$
% \State $\bm{M}_{trans}=[[~1, 0, {dx}~],~[~0, 1, {dy}~]]$
% \State $\bar{\bm{S}}_{tg}=\mathtt{WarpAffine}(\bm{S}_{rf}, \bm{M}_{trans}, \bm{S}_{rf}.shape)$
% \State {\bf Output:} Aligned Target Skeleton $\bar{\bm{S}}_{tg}$  
% %\\ 
% \end{algorithmic}
% \end{algorithm}


\begin{figure*}[t!]
\begin{center}
\includegraphics[width=0.98\linewidth]{editing_result.pdf}
\end{center}
\vspace{-0.55cm}
   \caption{Motion editing results of our MotionEditor. More examples can be found in the supplementary material and anonymous website.}
\label{fig:editing_result}
\vspace{-0.4cm}
\end{figure*}


\subsection{Skeleton Signal Alignment}
\label{sec: skeleton_alignment}
Given the source and reference videos, there always exists a gap between the source and the target protagonists due to different sizes and coordinated positions. The discrepancy may affect the performance of editing. Therefore, we propose an alignment algorithm for addressing this issue. 

Our algorithm contains two steps, namely a resizing operation and a translation operation.
Concretely, given the source video $\bm{X}_{sr}$ and a reference video $\bm{X}_{rf}$, we first extract the source skeleton $\bm{S}_{sr}$ and a foreground mask $\bm{M}_{sr}$, as well as the reference skeleton $\bm{S}_{rf}$ and its mask $\bm{M}_{rf}$, using off-the-shelf models.
We then perform edge detection on the masks to obtain rectangular outlines of the foreground.
Based on the area of two rectangular outlines, we scale $\bm{S}_{rf}$ to the same size as the source.
Regarding the foreground position, we calculate the average coordinate of the foreground pixels in each mask, which denotes the center of the protagonist.
An offset vector is computed by calculating the difference between the two centers.
With this vector, we obtain an affine matrix for the translation operation, which is further applied to the resized reference skeleton.
Finally, the target skeleton $\bar{\bm{S}}_{tg}$ is generated.
% The alignment is described in Algorithm \ref{alg:alignment}.
The details of alignment are depicted in the supplementary material.


%Concretely, we first implement OpenPose Detector to source video and target video obtaining source skeletons $\mathbf{S}_{s}$ and target skeletons $\mathbf{S}_{t}$. 
%We also utilize an off-the-shelf person segmentation model on two videos to segment the protagonists in the videos for obtaining corresponding protagonists masks $\mathbf{M}_{s}$ and $\mathbf{M}_{t}$. 
%Second, we perform edge detection on the part with a value of 1 in the two masks to obtain the rectangular outlines of the protagonists in the masks and the coordinates of the upper left corner of the protagonists. 
%We scale the target skeleton to the same size as the source skeleton based on the area of the rectangular outline. 
%Third, we calculate the average value of the coordinates with a value of 1 in each mask to obtain the center of the protagonist. 
%We calculate the offset vector between the center coordinates of the source mask and the target mask to further obtain the affine matrix that projects the target skeleton to the source skeleton. 
%We project the protagonist position of the target skeleton to the position of the source skeleton based on the affine matrix. 
%The alignment process is described in Alignment \ref{alg:alignment}. 
%$\mathbf{P}_{S_{t}}$ and $\mathbf{P}_{M_{t}}$ refers to the protagonist in the $\mathbf{S}_{t}$ and $\mathbf{M}_{t}$ respectively. We denote $\mathtt{Seg}(\cdot)$ as an off-the-shelf person segmentation model. 
%The details of $\mathtt{Boundary}(\cdot)$ are depicted in the supplementary material. 




==> sec/5_experiments.tex <==
\section{Experiments}
\label{sec:method}



\subsection{Implementation Details}
Our proposed MotionEditor is based on the Latent Diffusion Model~\cite{rombach2022high} (Stable Diffusion). We evaluate our model on YouTube videos and videos from the TaichiHD~\cite{siarohin2019first} dataset, in which each video includes a protagonist of at least 70 frames. The resolution of frames is unified to $512\times 512$. We perform one-shot learning for the motion adapter for 300 steps with a constant learning rate of $3\times 10^{-5}$. We employ DDIM inversion~\cite{song2020denoising} and null-text optimization~\cite{mokady2023null} with classifier-free guidance~\cite{ho2022classifier} during inference. 
Due to the usage of DDIM inversion and null-text optimization, MotionEditor needs 10 minutes to perform motion editing for each video on a single NVIDIA A100 GPU.
%Our MotionEditor takes about 5 minutes for one-shot learning \xintong{training or inference?} to perform motion editing for each video on a single NVIDIA A100 GPU.

\subsection{Motion Editing Results}



We validate the motion editing superiority of our proposed MotionEditor extensively. Here, we demonstrate several cases in Figure \ref{fig:editing_result} and the rest of the cases are in the supplementary materials. 
% We chose four open wild dancing videos for motion editing in Figure \ref{fig:editing_result}, in which each colorful rounded rectangle block indicates one specific case. 
%The first row, the second row, and the third row refer to the source video, target video, and motion-edited video, respectively in each block. 
We can see that our MotionEditor can accomplish a wide range of motion editing while simultaneously preserving the original protagonist's appearance and background information. 

\begin{figure}[t!]
\begin{center}
\includegraphics[width=1\linewidth]{comparison.pdf}
\end{center}
\vspace{-0.3cm}
   \caption{Qualitative comparison between our MotionEditor and other state-of-the-art video editing models. 
   %(a), (b), (c), (d), (e), (f), (g), (h), (i), (j) indicates to source video, target video, LWG~\cite{liu2019liquid}, MRAA~\cite{siarohin2021motion}, Tune-A-Video~\cite{wu2023tune}, Follow-Your-Pose~\cite{ma2023follow}, ControlVideo~\cite{zhang2023controlvideo}, Masactrl~\cite{cao2023masactrl}, FateZero~\cite{qi2023fatezero}, our proposed MotionEditor. Best viewed in color.
   Source prompt: ``a girl in a black dress is dancing."
   Target prompt: ``a girl in a black dress is practicing tai chi."
   Our method exhibits accurate motion editing and appearance preservation.
   }
\label{fig:comparison_result}
\vspace{-0.2cm}
\end{figure}

\subsection{Comparison with State-of-the-Art Methods}
\textbf{Competitors.} We compare our MotionEditor against recent approaches to validate the superiority of our model. The competitors are depicted as follows: 
(1) Models based on GANs for human motion transfer, including LWG~\cite{liu2019liquid} that disentangles the pose and shape, and MRAA~\cite{siarohin2021motion} that learns semantic object parts.
%Previous human motion transfer GAN models: LWG~\cite{liu2019liquid} utilizes a 3D body mesh recovery module to disentangle the pose and shape. MRAA~\cite{siarohin2021motion} proposes PCA-based region motion representation for capturing objective parts.
% (2) Tune-A-Video~\cite{wu2023tune} is a one-shot learning-based video editing model that can be equipped with conditional T2I models (Controlnet~\cite{zhang2023adding}) and inflated Stable Diffusion for handling controllable video generation task. 
(2) Tune-A-Video~\cite{wu2023tune}, which inflates Stable Diffusion in a one-shot learning manner. 
% (3) Follow-Your-Pose~\cite{ma2023follow} proposes a spatial pose adapter for pose-guided video generation which plays the same role as the original Controlnet~\cite{zhang2023adding}. 
(3) Follow-Your-Pose~\cite{ma2023follow}, which proposes a spatial pose adapter for pose-guided video generation.
% (4) ControlVideo~\cite{zhang2023controlvideo} designs fully cross-frame attention and interleaved-frame smoother which attempts to stitch video frames into one large image for transferring original prior knowledge of Stable Diffusion from the image domain to the video domain. 
(4) ControlVideo~\cite{zhang2023controlvideo}, which designs fully cross-frame attention, attempting to stitch video frames into one large image. 
(5) MasaCtrl~\cite{cao2023masactrl}, which conducts mask-guided mutual self-attention fusion, in which the masks are derived from text cross attention. 
(6) FateZero~\cite{qi2023fatezero}, which designs inversion attention fusion for retaining source structure. 
It is worth noting that Tune-A-Video and Masactrl are equipped with a conditional T2I model (\emph{i.e.} ControlNet) for controllable video editing.
We also combine FateZero with ControlNet to enable pose-guided editing.
More details on implementation are depicted in the supplementary material.



\textbf{Qualitative results.} 
% Given source prompt "a girl in black dress is dancing", target prompt "a girl in black dress is practicing tai chi", source video, and target video, 
We conduct a qualitative comparison of our MotionEditor against several competitors in Fig. \ref{fig:comparison_result}. The results of LWG~\cite{liu2019liquid} and MRAA~\cite{siarohin2021motion} are provided in the supplementary material. By analyzing the results, we have the following observations: 
% (1) Previous motion transfer GAN~\cite{creswell2018generative} models LWG~\cite{liu2019liquid} and MRAA~\cite{siarohin2021motion} fail to preserve original appearance or transfer target motion to source video. 
(1) Tune-A-Video~\cite{wu2023tune}, ControlVideo~\cite{zhang2023controlvideo}, Masactrl~\cite{cao2023masactrl} and FateZero~\cite{qi2023fatezero} demonstrate capabilities in editing motion to a certain extent.
Nevertheless, their edited videos exhibit a considerable degree of ghosting, manifested as overlapping frames of the protagonist's heads and legs. 
%transfer the motion information to a certain degree. However, their edited video contains a significant amount of ghosting, such as overlapping frames of girl's heads and legs. 
(2) Follow-Your-Pose~\cite{ma2023follow} fails to perform motion editing and preserve the source appearance. The ghosting effect also exists in the result. The plausible reason is that it has difficulties handling the motion conflict between inverted noise and input reference pose.
%its spatial pose adapter only focuses on spatial frame-wise pose representations, ignoring temporal motion modeling. 
% (3) Tune-A-Video~\cite{wu2023tune} and ControlVideo~\cite{zhang2023controlvideo} both have dramatic background and protagonist appearance changes compared with other competitors. Due to their single-branch architectural constraints, they are unable to interact with the original video features when additional pose conditions are introduced. This leads to a gradual loss of the original video's geometric structure and protagonist appearance features as the denoising phase progresses with increasing steps. 
(3) Tune-A-Video~\cite{wu2023tune} and ControlVideo~\cite{zhang2023controlvideo} both have dramatic appearance changes, \emph{e.g.}, hairstyle, texture of clothes and background. 
Due to the constraint of a single-branch architecture, they are unable to interact with the original video features when additional pose conditions are introduced. 
This leads to a gradual loss of the source appearance along with the increasing denoising steps. 
(4) Masactrl~\cite{cao2023masactrl} generates an excessive amount of blurry noise. 
% Masactrl executes text cross-attention masks guided attention fusion for decoupling the self-attention map during the editing process. 
The possible reason is that the masks generated by cross attention maps are unreliable and inconsistent across time, thus introducing blurring noise to the result.
%temporal inconsistency of masks results in the introduction of a significant amount of noise during the denoising process. 
(5) The edited result of FateZero~\cite{qi2023fatezero} shows overlapping frames of the protagonist's legs. 
It demonstrates that the attention fusion strategy in FateZero may not be suitable for motion editing. 
(6) Finally, our MotionEditor can effectively perform motion editing while preserving the original background and appearance compared with previous approaches, highlighting its great potential.

\begin{table}[t!]\small
\caption{Quantitative comparisons on 20 in-the-wild cases. L-S, L-N, and L-T indicate LPIPS-S, LPIPS-N, LPIPS-T respectively. 
% LPIPS refers to Learned Perceptual Image Patch Similarity.
%~\cite{zhang2018perceptual}
}
\vspace{-0.1in}
\begin{center}
\renewcommand\arraystretch{1.1}
\scalebox{0.9}{
\begin{tabular}{lcccc}
\toprule
Method           & CLIP ($\uparrow$)           & L-S ($\downarrow$)       & L-N ($\downarrow$)        & L-T ($\downarrow$)       \\ \midrule
LWG~\cite{liu2019liquid}              & 25.35          & 0.431          & 0.194          & 0.203          \\
MRAA~\cite{siarohin2021motion}             & 26.80          & 0.462          & 0.269          & 0.353          \\
Tune-A-Video~\cite{wu2023tune}     & 27.71          & 0.345          & 0.169          & 0.157          \\
Follow-Your-Pose~\cite{ma2023follow} & 26.55          & 0.337          & 0.144          & 0.183          \\
ControlVideo~\cite{zhang2023controlvideo}     & 26.87          & 0.428          & 0.228          & 0.311          \\
MasaCtrl~\cite{cao2023masactrl}         & 27.14          & 0.372          & 0.236          & 0.177          \\
FateZero~\cite{qi2023fatezero}         & 28.07          & 0.308          & 0.176          & 0.124          \\ \midrule
MotionEditor     & \textbf{28.86} & \textbf{0.273} & \textbf{0.124} & \textbf{0.082} \\ \bottomrule
\end{tabular}
}
\end{center}
\label{table:quantitative_comparisons}
\vspace{-0.2in}
\end{table}


% \begin{table}[t]\small
% \caption{User preference depicted as a percentage. \textsuperscript{*} refers to the preference proportion of MotionEditor. M-A, A-A and T-A indicate motion alignment, appearance alignment, and textual alignment, respectively.}
% \vspace{-0.1in}
% \begin{center}
% \renewcommand\arraystretch{1.1}
% \scalebox{0.81}{
% \begin{tabular}{lmmm}
% \toprule
% Method           & M-A & A-A & T-A \\ \midrule
% LWG~\cite{liu2019liquid}              & 8.1\%/\textbf{91.9\%\textsuperscript{*}}       & 4.3\%/\textbf{95.7\%\textsuperscript{*}}           & 10.0\%/\textbf{90.0\%\textsuperscript{*}}       \\
% MRAA~\cite{siarohin2021motion}             & 5.2\%/\textbf{94.8\%\textsuperscript{*}}       & 1.6\%/\textbf{98.4\%\textsuperscript{*}}           & 7.4\%/\textbf{92.6\%\textsuperscript{*}}        \\
% Tune-A-Video~\cite{wu2023tune}     & 12.4\%/\textbf{87.6\%\textsuperscript{*}}      & 9.2\%/\textbf{90.8\%\textsuperscript{*}}           & 20.8\%/\textbf{79.2\%\textsuperscript{*}}       \\
% Follow-Your-Pose~\cite{ma2023follow} & 3.7\%/\textbf{96.3\%\textsuperscript{*}}       & 15.0\%/\textbf{85.0\%\textsuperscript{*}}          & 15.4\%/\textbf{84.6\%\textsuperscript{*}}       \\
% ControlVideo~\cite{zhang2023controlvideo}     & 5.9\%/\textbf{94.1\%\textsuperscript{*}}       & 1.2\%/\textbf{98.8\%\textsuperscript{*}}           & 14.0\%/\textbf{86.0\%\textsuperscript{*}}       \\
% MasaCtrl~\cite{cao2023masactrl}         & 10.6\%/\textbf{89.4\%\textsuperscript{*}}      & 5.4\%/\textbf{94.6\%\textsuperscript{*}}           & 12.2\%/\textbf{87.8\%\textsuperscript{*}}       \\
% FateZero~\cite{qi2023fatezero}         & 21.1\%/\textbf{78.9\%\textsuperscript{*}}      & 25.5\%/\textbf{74.5\%\textsuperscript{*}}          & 25.3\%/\textbf{74.7\%\textsuperscript{*}}       \\ \bottomrule
% \end{tabular}
% }
% \end{center}
% \label{table:user_study}
% \vspace{-0.2in}
% \end{table}



\textbf{Quantitative results.} To the best of our knowledge, there is still no widely recognized metric for evaluating the performance of video editing. 
In this paper, we conduct quantitative comparisons against previous approaches through several perceptual metrics~\cite{zhang2018perceptual} and a user study on edited videos.
%motion corresponding consistency and user study of edited videos. 
%We conduct three metrics for measuring consistency: 
The detailed metrics are as follows: (1) CLIP score~\cite{radford2021learning}: Target textual faithfulness. (2) LPIPS-S: Learned Perceptual Image Patch Similarity (LPIPS)~\cite{zhang2018perceptual} between edited frames and source frames. (3) LPIPS-N: LPIPS between edited neighboring frames. 
(4) LPIPS-T: We split a long video into two segments. The first segment is used for the source, while the second segment is for the reference. We compute LPIPS between the edited video and the second segment. The results are shown in Table \ref{table:quantitative_comparisons}.
We observe that MotionEditor surpasses the competitors by a large margin.
% In terms of motion corresponding consistency, we utilize OpenPose Detector on each edited frame and each target frame to obtain each edited skeleton and each target skeleton. We calculate the Euclidean distance between edited key points and target key points. The motion similarity is obtained by normalizing and averaging the distances. It is worth noting that the target skeleton is aligned with the edited skeleton before calculating motion similarity. 

\begin{table}[t!]\small
\caption{User preference ratio of MotionEditor when comparing with each method. Higher indicates the users prefer more to our MotionEditor. M-A, A-A and T-A indicate motion alignment, appearance alignment, and textual alignment, respectively.}
\vspace{-0.1in}
\begin{center}
\renewcommand\arraystretch{1.1}
\scalebox{0.95}{
\begin{tabular}{lccc}
\toprule
Method           & M-A & A-A & T-A \\ \midrule
LWG~\cite{liu2019liquid}              & 91.9\%       & 95.7\%           & 90.0\%       \\
MRAA~\cite{siarohin2021motion}             & 94.8\%       & 98.4\%           & 92.6\%        \\
Tune-A-Video~\cite{wu2023tune}     & 87.6\%      & 90.8\%           & 79.2\%       \\
Follow-Your-Pose~\cite{ma2023follow} & 96.3\%       & 85.0\%          & 84.6\%       \\
ControlVideo~\cite{zhang2023controlvideo}     & 94.1\%       & 98.8\%           & 86.0\%       \\
MasaCtrl~\cite{cao2023masactrl}         & 89.4\%      & 94.6\%           & 87.8\%       \\
FateZero~\cite{qi2023fatezero}         & 78.9\%      & 74.5\%          & 74.7\%      \\ \bottomrule
\end{tabular}
}
\end{center}
\label{table:user_study}
\vspace{-0.2in}
\end{table}

We also conduct a user study to evaluate the human preference between our method and the competitors.
For each case, participants are first presented with the source and target videos, as well as the prompts.
We then show two motion-edited videos; one is generated by our method and the other is from a competitor, in random order.
Participants are asked to answer the following questions: ``which one has better motion alignment with reference", 
``which one has better appearance alignment with source", and
``which one has better content alignment with the prompt."
The total number of cases is 20, and the participants are mainly university students.
The results in Table~\ref{table:user_study} show that our method is far ahead of other methods in terms of subjective evaluation.
%For the User Study, we first present a source video and a target video. we then present the motion-edited videos by our method and other previous approaches in random order, asking the voters to answer the questions "Which one has better motion alignment with target video?" and "Which one has better appearance alignment with source video?". In terms of textual faithfulness, we additionally present a target prompt and ask voters to answer the question "Which one has better content alignment with prompt description?". We conducted a user study on 20 cases and the voters were mainly students in university. The result is in Table \ref{table:user_study}.

\begin{figure}[t!]
\begin{center}
\includegraphics[width=1\linewidth]{ablation.pdf}
\end{center}
\vspace{-0.3cm}
   \caption{Ablations on core components of MotionEditor.
   Rows in the figure are: (a) source, (b) reference, (c) \textit{w/o} CS Attention, (d) \textit{w/o} cross attention in motion adapter, (e) \textit{w/o} motion adapter, (f) \textit{w/o} high-fidelity attention injection, (g) \textit{w/o} skeleton alignment, and (h) MotionEditor.
   %(a), (b), (c), (d), (e), (f), (g), (h) refers to source video, target video, model \textit{w/o} C-Sparse Attention, model \textit{w/o} Content-Aware Cross Attention, model \textit{w/o} Content-Aware Motion Adapter, model \textit{w/o} Two Stream Attention Injection Mechanism, model \textit{w/o} Skeleton Signals Alignment and MotionEditor. 
   Source prompt: ``A girl is dancing." Target prompt: ``A girl is practicing tai chi."}
\label{fig:ablation}
\vspace{-0.2cm}
\end{figure}

\subsection{Ablation Study}
To validate the importance of the core components in MotionEditor, we conduct an ablation study. The results are illustrated in Fig. \ref{fig:ablation}. It is worth noting that we replace our proposed CS Attention with the previous Sparse Attention~\cite{wu2023tune} in (c). 
The results in row (c) indicate that Sparse Attention attempts to force the frames to be aligned with the first frame, resulting in unreliable motion. 
% Model \textit{w/o} Temporal-Latent-aware Motion Adapter fails to execute motion transferring and background preservation. It demonstrates that the original Controlnet has weak constraints on the motion of video frames without additional temporal-aware modeling and latent-aware modeling. 
Rows (d) and (e) both fail to accomplish motion editing and background preservation. It demonstrates that the original ControlNet has weak constraints on the motion without additional content-aware modeling. It also forces the model to retain background information.
% Model \textit{w/o} Two Stream Attention Injection Mechanism lacks the original background details as the girl's clothes and the road sign behind her are changed or disappeared. It validates that our proposed mechanism can promote the model to preserve the source background information and the protagonist's appearance. 
In row (f), model \textit{w/o} high-fidelity attention injection loses the original background details as the road sign behind the girl has disappeared. It validates that our proposed mechanism can promote the model to preserve the source background. 
% Model \textit{w/o} Skeleton Signals Alignment suffers from background and protagonist appearance changing due to the misalignment between source skeletons and target skeletons. The misalignment of the skeleton may potentially introduce additional unexpected noise to the content latent destroying its original data distribution and resulting in failure of denoising. The above ablation results demonstrate that our core components certainly contribute to the promising motion editing capacity of MotionEditor.
Model \textit{w/o} skeleton alignment suffers from appearance change due to the misalignment, as in row (g). 
The misalignment of the skeletons may potentially introduce unexpected noise to the content latent, thus destroying source data distribution. The above ablation results demonstrate that our core components certainly contribute to the promising motion editing capability of MotionEditor.

==> sec/6_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion} In this paper, we proposed MotionEditor for tackling video motion editing challenges, which is rated as high-level video editing compared with previous video attribute editing. 
% Video motion editing aims to transfer motion from the target video to the source video while preserving the source background and protagonist's appearance.
% We take the first attempt to explore the video motion editing diffusion model.
To enhance the motion controllability, a content-aware motion adapter was designed to build up a relationship with the source content, enabling seamless motion editing as well as temporal modeling.
%enable ControlNet to capture temporal motion and build up a correlated relationship with content. 
We further proposed a high-fidelity attention injection for preserving the source appearance of the background and protagonist. 
To alleviate the misalignment problem of skeleton signals, we presented a simple yet effective skeleton alignment to normalize the target skeletons. 
%Extensive experiments indicate the superiority of our MotionEditor in the video motion editing task. 
To our knowledge, MotionEditor is the first diffusion model to explore the video motion editing task, encouraging more future studies in this challenging scenario.
% To our knowledge, MotionEditor is the first model to explore video motion editing tasks. 
